Benchmarking Smoothness and Reducing High-Frequency Oscillations in Continuous Control Policies

Reinforcement learning (RL) policies are prone to high-frequency oscillations, especially undesirable when deploying to hardware in the real-world. In this paper, we identify, categorize, and compare methods from the literature that aim to mitigate high-frequency oscillations in deep RL. We define two broad classes: loss regularization and architectural methods. At their core, these methods incentivize learning a smooth mapping, such that nearby states in the input space produce nearby actions in the output space. We present benchmarks in terms of policy performance and control smoothness on traditional RL environments from the Gymnasium and a complex manipulation task, as well as three robotics locomotion tasks that include deployment and evaluation with real-world hardware. Finally, we also propose hybrid methods that combine elements from both loss regularization and architectural methods. We find that the best-performing hybrid outperforms other methods, and improves control smoothness by 26.8% over the baseline, with a worst-case performance degradation of just 2.8%.

==> Tables/gymnasium_specific_parameter.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Method}                 & \textbf{Parameter}    & \textbf{Value} \\ \hline
\multirow{3}{*}{CAPS}           & $\sigma$              & 0.1            \\ \cline{2-3} 
                                & $\lambda_T$           & 0.1            \\ \cline{2-3} 
                                & $\lambda_S$           & 0.5            \\ \hline

\multirow{3}{*}{L2C2}           & $\sigma$              & 1.0            \\ \cline{2-3} 
                                & $\underline{\lambda}$ & 0.01           \\ \cline{2-3}
                                & $\overline{\lambda}$  & 1.0            \\ \cline{2-3}
                                & $\beta$               & 0.1            \\ \hline
                               
\multirow{7}{*}{LipsNet}        & Weight $\lambda$      & 0.1                       \\ \cline{2-3} 
                                & $\epsilon$             & 0.0001                    \\ \cline{2-3} 
                                & Initial Lipschitz constant $K_\text{init}$ & 1.0  \\ \cline{2-3} 
                                & Hidden layers in $f(x)$   & {[}64, 64{]}          \\ \cline{2-3} 
                                & Activation in $f(x)$      & ELU                   \\ \cline{2-3} 
                                & Hidden layers in $K(x)$   & {[}32{]}              \\ \cline{2-3} 
                                & Activation in $K(x)$      & Tanh                  \\ \hline

\multirow{2}{*}{Liu-Lipschitz}  & Weight $\lambda$           & $1 \times 10^{-6}$   \\ \cline{2-3} 
                                & Initial Lipschitz constant & 10.0                 \\ \hline

\end{tabular}
\caption{Hyperparameters for the methods investigated in our work for the Gymnasium environments. The same hyperparameters are used for every environment.}
\label{tab:gymnasium_method_specific_parameter_table}
\end{table}

==> Tables/imitation_ppo_parameter_table.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Parameter}   & \textbf{Value}            \\ \hline
Number of Environments       & $4096$  \\ \hline
Horizon Length       & $24$  \\ \hline
Batch size           & $98304$  \\ \hline
Learning rate        & $3 \times 10^{-4}$        \\ \hline
Clip rate            & $0.2$                     \\ \hline
KL-divergence        & $0.008$                   \\ \hline
Entropy coefficient  & $0.00$                    \\ \hline
Discount factor      & $0.95$                    \\ \hline
GAE discount factor  & $0.95$                    \\ \hline

\end{tabular}
\caption{PPO hyperparameters for training the \textbf{Locomotion - Motion Imitation} environment.}
\label{tab:imitation_ppo_parameter_table}
\end{table}

==> Tables/imitation_reward_table.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Reward Term}      & \textbf{Value}        \\ \hline
Weight - DoF Position              & $0.5$                  \\ \hline
Weight - DoF Velocity              & $0.05$                 \\ \hline
Weight - End-effector Position     & $0.2$                  \\ \hline
Weight - Root Position             & $0.15$                 \\ \hline
Weight - Root Velocity             & $0.1$                  \\ \hline
Scale - DoF Position        & $5.0$                  \\ \hline
Scale - DoF Velocity        & $0.1$                  \\ \hline
Scale - End-effector        & $40.0$                 \\ \hline
Scale - Root position       & $20.0$                 \\ \hline
Scale - Root velocity       & $2.0$                  \\ \hline
\end{tabular}
\caption{Reward terms for \textbf{Locomotion - Motion Imitation} environment.}
\label{tab:imitation_reward_table}
\end{table}

==> Tables/imitation_specific_parameter.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Method}                 & \textbf{Parameter}    & \textbf{Value} \\ \hline
\multirow{3}{*}{CAPS}           & $\sigma$              & 0.2            \\ \cline{2-3} 
                                & $\lambda_T$           & 0.01           \\ \cline{2-3} 
                                & $\lambda_S$           & 0.05           \\ \hline

\multirow{3}{*}{L2C2}           & $\sigma$              & 1.0            \\ \cline{2-3} 
                                & $\underline{\lambda}$ & 0.01           \\ \cline{2-3}
                                & $\overline{\lambda}$  & 1.0            \\ \cline{2-3}
                                & $\beta$               & 0.1            \\ \hline
                               
\multirow{7}{*}{LipsNet}         & Weight $\lambda$      & $1 \times 10^{-3}$       \\ \cline{2-3} 
                                & $\epsilon$             & 0.0001                   \\ \cline{2-3} 
                                & Initial Lipschitz constant $K_\text{init}$ & 1.0  \\ \cline{2-3} 
                                & Hidden layers in $f(x)$   & {[}512, 256{]}        \\ \cline{2-3} 
                                & Activation in $f(x)$      & ELU                   \\ \cline{2-3} 
                                & Hidden layers in $K(x)$   & {[}32{]}              \\ \cline{2-3} 
                                & Activation in $K(x)$      & Tanh                  \\ \hline

\multirow{2}{*}{Liu-Lipschitz}  & Weight $\lambda$           & $1 \times 10^{-6}$   \\ \cline{2-3} 
                                & Initial Lipschitz constant & 10.0                 \\ \hline

\multirow{3}{*}{Butterworth Low-pass Filter} & Order                 & 2            \\ \cline{2-3} 
                                             & Cutoff Frequency        & 4.0 Hz       \\ \hline
\end{tabular}
\caption{Hyperparameters for the methods investigated in our work for the \textbf{Locomotion - Motion Imitation} environment.}
\label{tab:imitation_method_specific_parameter_table}
\end{table}

==> Tables/velocity_method_specific_parameter_table.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Method}                & \textbf{Parameter}    & \textbf{Value} \\ \hline
\multirow{3}{*}{CAPS}          & $\sigma$              & 0.2            \\ \cline{2-3} 
                               & $\lambda_T$           & 0.01           \\ \cline{2-3} 
                               & $\lambda_S$           & 0.05           \\ \hline
\multirow{2}{*}{L2C2}          & $\lambda_\pi$         & 1.0            \\ \cline{2-3} 
                               & $\lambda_V$           & 0.1            \\ \hline
\multirow{4}{*}{LipsNet}       & Weight $\lambda$      & $1 \times 10^{-3}$          \\ \cline{2-3} 
                               & Initial Lipschitz constant $K_\text{init}$               & 1.0            \\ \cline{2-3} 
                               & Hidden layers in $K(x)$  & {[}32{]}    \\ \cline{2-3} 
                               & Activation in $K(x)$  & Tanh           \\ \hline
\multirow{2}{*}{Liu-Lipschitz} & Weight $\lambda$      & $1 \times 10^{-6}$    \\ \cline{2-3} 
                               & Initial Lipschitz constant & 10.0             \\ \hline
\multirow{2}{*}{Butterworth Low-pass Filter}   & Order      & 2            \\ \cline{2-3} 
                                               & Cutoff Frequency   & 4.0 Hz            \\ \hline
\end{tabular}
\caption{Method-specific hyper-parameters for \textbf{Locomotion - Velocity Controller} environment.}
\label{tab:velocity_method_specific_parameter_table}
\end{table}

==> Tables/velocity_ppo_parameter_table.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Parameter}   & \textbf{Value}     \\ \hline
Batch size           & $98304 (4096 \times 24)$  \\ \hline
Learning rate        & $5 \times 10^{-4}$        \\ \hline
Clip rate            & $0.2$              \\ \hline
KL-divergence        & $0.01$             \\ \hline
Entropy coefficient  & $0.02$             \\ \hline
Discount factor      & $0.99$             \\ \hline
GAE discount factor  & $0.95$             \\ \hline

\end{tabular}
\caption{PPO hyper-parameters for training the \textbf{Locomotion - Velocity Controller} environment.}
\label{tab:velocity_ppo_parameter_table}
\end{table}

==> Tables/velocity_reward_table.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Reward Term}      & \textbf{Weight}        \\ \hline
Linear velocity tracking  & $0.02$                 \\ \hline
Angular velocity tracking & $0.01$                 \\ \hline
Linear velocity penalty   & $-0.04$                \\ \hline
Angular velocity penalty  & $-0.001$               \\ \hline
Joint acceleration        & $-5 \times 10^{-9}$    \\ \hline
Joint position limit      & $-0.2$                 \\ \hline
Feet air time             & $0.03$                 \\ \hline
Collisions                & $0.02$                 \\ \hline
Base height               & $-0.2$                 \\ \hline
Orientation               & $-0.02$                \\ \hline
Torques                   & $-4 \times 10^{-6}$    \\ \hline
\end{tabular}
\caption{Reward terms for \textbf{Locomotion - Velocity Controller} environment.}
\label{tab:velocity_reward_table}
\end{table}
